Expressive Text-to-Image Generation with Rich Text

Plain text has become a prevalent interface for text-to-image synthesis. However, its limited customization options hinder users from accurately describing desired outputs. For example, plain text makes it hard to specify continuous quantities, such as the precise RGB color value or importance of each word. Furthermore, creating detailed text prompts for complex scenes is tedious for humans to write and challenging for text encoders to interpret. To address these challenges, we propose using a rich-text editor supporting formats such as font style, size, color, and footnote. We extract each word's attributes from rich text to enable local style control, explicit token reweighting, precise color rendering, and detailed region synthesis. We achieve these capabilities through a region-based diffusion process. We first obtain each word's region based on attention maps of a diffusion process using plain text. For each region, we enforce its text attributes by creating region-specific detailed prompts and applying region-specific guidance, and maintain its fidelity against plain-text generation through region-based injections. We present various examples of image generation from rich text and demonstrate that our method outperforms strong baselines with quantitative evaluations.

==> figures/ablation2.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth, trim=0 0 0 0, clip]{figures/images/ablation2.pdf}
    \caption{\textbf{Mean vs. max attention values for token maps.} We show that taking the mean across tokens of the span can lead to inaccurate \textit{token maps}.}
    \label{fig:ablation2}
\end{figure}

% \vspace{-0.1cm}

==> figures/composed_style.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth, trim=0 0 0 0, clip]{figures/images/composed_style_main.pdf}
    \caption{\textbf{Composed-based method.} We apply InstructPix2Pix~\cite{brooks2022instructpix2pix} on two regions separately and compose the results using token maps. The generation contains sharp changes and artifacts at the boundary areas. We show three random seeds.}
    \label{fig:composed_baseline}
    % \vspace{-10pt}
\end{figure}


==> figures/limitation1.tex <==
\begin{figure}[t]
    \centering
    % \vspace{-0.4cm}
    \includegraphics[width=\linewidth, trim=0 0 0 0, clip]{figures/images/limitation1.pdf}
    \caption{\textbf{Failure cases.} The color leaks to the background due to the inaccurate ``shirt'' token map.}
    \label{fig:limitation1}
    % \vspace{-15pt}
\end{figure}


==> figures/teaser.tex <==
\begin{strip}
\vspace{-2.9cm}
\centering
% \captionsetup{type=figure}
\includegraphics[width=\linewidth,trim=0 0 0 0, clip]{figures/images/teaser.pdf}
\captionof{figure}{{\bf Plain text (left image) vs. Rich text (right image).} Our method allows a user to describe an image using a rich text editor that supports various text attributes like font family, size, color, and footnote. Given these text
attributes extracted from rich-text prompts, our method enables precise control of text-to-image synthesis regarding colors, styles, and object details compared to plain text. }
\label{fig:teaser}
\end{strip}
